Global Weather for the Astronomical Observatories

Astronomical sites occupying observing instruments have to be selected according to many factors. Among these factors, geographic location of the site and quality of atmosphere above the site play an important role in the decision process. The following factors were chosen to create layers at their geographic locations (observatories: 1905 northern, 235 southern) from the \href{https://www.astrogis.org}{astroGIS database}: CC (cloud coverage), PWV (precipitable water vapor), AOD (atmospheric optical depth), VWV (vertical wind velocity) and HWV (horizontal wind velocity). In order to estimate astronomical importance of geographic location of the sites and quality of airmass above the sites, DEM (digital elevation model) and LAT (latitude of observatory location) layers were also included. Two periodic variations have been produced from these factors: monthly and annual averages. In addition to the variations or trends a complete statistical analysis was carried out for all factors to investigate the potential correlations between the factors: There is a clear difference between northern and southern hemispheres. Exchange of meteorological seasons between hemispheres are also compliant within factors. The geographical locations of most of the observatories found to be "not suitable": On the average, DEM is low (550 m), CC is high (70\%) and PWV is high (14 mm). There seems to be no apparent long-term variations and/or patterns in all factors. We once again confirm the common expectation of astronomy: \textit{as DEM increases astronomical conditions get better} (CC, PWV and AOD gets lower values). All the results will be made available online through astroGIS database.

==> inc/old/w-fig2.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{@{}c@{}c@{}}
    \includegraphics[height=4.25cm]{fig/fig2/monthly_CC_N.png}       &
    \includegraphics[height=4.25cm]{fig/fig2/monthly_CC_S.png}       \\
    \includegraphics[height=4.25cm]{fig/fig2/monthly_PWV_N.png}      &
    \includegraphics[height=4.25cm]{fig/fig2/monthly_PWV_S.png}      \\
    \includegraphics[height=4.25cm]{fig/fig2/monthly_AOD_10K_S.png}  &
    \includegraphics[height=4.25cm]{fig/fig2/monthly_AOD_10K_N.png}  \\
    \includegraphics[height=4.25cm]{fig/fig2/monthly_VVWS_N.png}     &
    \includegraphics[height=4.25cm]{fig/fig2/monthly_VVWS_S.png}     \\
    \includegraphics[height=4.25cm]{fig/fig2/monthly_200hPAWS_N.png} &
    \includegraphics[height=4.25cm]{fig/fig2/monthly_200hPAWS_S.png} \\
    \end{tabular}
\caption{%
Monthly averages for northern (left panel) and southern (right panel) observatories for layers CC, PWV, AOD, WS1, WS2, from top to bottom, respectively. XXXXXX TALK ABOUT TRENDS AND HEMISPHERE DIFFERENCE%
}
\label{F:monthly}
\end{figure*}

==> inc/old/w-fig3.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{@{}c@{}c@{}}
    \includegraphics[height=4.25cm]{fig/fig3/yearly_CC_N.png}        &
    \includegraphics[height=4.25cm]{fig/fig3/yearly_CC_S.png}        \\
    \includegraphics[height=4.25cm]{fig/fig3/yearly_PWV_N.png}       &
    \includegraphics[height=4.25cm]{fig/fig3/yearly_PWV_S.png}       \\
    \includegraphics[height=4.25cm]{fig/fig3/yearly_AOD_10K_N.png}   &
    \includegraphics[height=4.25cm]{fig/fig3/yearly_AOD_10K_S.png}   \\
    \includegraphics[height=4.25cm]{fig/fig3/yearly_VVWS_N.png}      &
    \includegraphics[height=4.25cm]{fig/fig3/yearly_VVWS_S.png}      \\
    \includegraphics[height=4.25cm]{fig/fig3/yearly_200hpaWS_N.png}  &
    \includegraphics[height=4.25cm]{fig/fig3/yearly_200hpaWS_S.png}  \\
    \end{tabular}
\caption{%
Yearly averages for northern (left panel) and southern (right panel) observatories for layers CC, PWV, AOD, WS1, WS2, from top to bottom, respectively. XXXXXX TALK ABOUT TRENDS AND HEMISPHERE DIFFERENCE%
}
\label{F:yearly}
\end{figure*}

==> inc/old/w-fig6.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{@{}c@{}c@{}}
    \includegraphics[height=6.25cm]{fig/fig6/hist-dem.eps}   &
    \includegraphics[height=6.25cm]{fig/fig6/hist-cc.eps}    \\
    \includegraphics[height=6.25cm]{fig/fig6/hist-pwv.eps}   &
    \includegraphics[height=6.25cm]{fig/fig6/hist-aod.eps}   \\
    \includegraphics[height=6.25cm]{fig/fig6/hist-vv.eps}    &
    \includegraphics[height=6.25cm]{fig/fig6/hist-200.eps}   \\
    \end{tabular}
\caption{%
    Histogram plot of yearly averages for observatories of layers DEM(upper left), CC(upper right), PWV(middle left), AOD(middle right), WS1(bottom left), WS2 (bottom right), respectively, from top to bottom. Bin size is given upper right of the plot. The histogram also includes the mean except for DEM and WS1, $\mu$ (solid line), $\mu-1\sigma$ (dotted line), $\mu-2\sigma$ (dashed line), $\mu-3\sigma$ (dash-dotted line). The signs between $\mu$ and $\sigma$ are + for DEM $\pm$. Statistical values are given in Table \ref{T:tab6}. %
}
\label{F:hist}
\end{figure*}

==> inc/old/w-special_obs.tex <==
\begin{figure*}
\centering
\begin{tabular}{@{}c@{}c@{}}
\includegraphics[height=5.25cm]{fig/fig8/CATANIA_PWV_YEAR.png} & 
\includegraphics[height=5.25cm]{fig/fig8/CONCELL_YEAR.png}
\\
    \end{tabular}
\caption{
The two observatories with the highest R$^{2}$ values in annual trend analyzes for 2141 observatories: R$^{2}$ = 0.70 for the annual average cloudiness at the Observatorio Astronomico de Consell Observatory in Spain, and the annual average at the Astrophysical Observatory in Catania R $^{2}$ = 0.86 for precipitable water vapor.
}
\label{F:special_obs}
\end{figure*}




==> inc/old/w-tab4_4.tex <==
\begin{table*}
    \caption{%
    Linear regressions obtained from annual changes for CC, PWV, AOD, WS1, 200hPAWS layers.
    Each layer contains two columns: the slope and quality of the linear regression.%
}
    \centering
    \begin{tabular}{lrrrrrrrrrr}
    \hline \hline
Site
& \multicolumn{2}{c}{CC [\%]}
& \multicolumn{2}{c}{PWV [mm]}
& \multicolumn{2}{c}{AOD [value]}
& \multicolumn{2}{c}{WS2[m s$^{-1}$]}
& \multicolumn{2}{c}{WS1 [Pa s$^{-1}$]}
\\

& \multicolumn{1}{c}{S}
& \multicolumn{1}{c}{R$^{2}$}
& \multicolumn{1}{c}{S}
& \multicolumn{1}{c}{R$^{2}$}
& \multicolumn{1}{c}{S}
& \multicolumn{1}{c}{R$^{2}$}
& \multicolumn{1}{c}{S}
& \multicolumn{1}{c}{R$^{2}$}
& \multicolumn{1}{c}{S}
& \multicolumn{1}{c}{R$^{2}$}
\\ 
\hline
SAAO	&	-0.17&0.10	&	0.00&0.00	&	0.00	&	0.15	&	0.06 &0.18	&	0.00&0.10	\\
CPO	    &	-0.07&0.01	&	0.01&0.01	&	-6.19	&	0.27	&	0.06&0.14	&	0.01&0.48	\\
CTIO	&	-0.12&0.03	&	0.02&0.01	&	0.37	&	0.54	&   0.06&0.14	&	0.02&0.00	\\
LCO	    &	0.05&0.00	&	-0.07&0.14	&	-0.01	&	0.00	&   0.07&0.16	&	0.03&0.03	\\
CA	    &	0.17&0.16	&	-0.03&0.10	&	0.10	&	0.01	&	0.06&0.10	&	0.04&0.10	\\
PO	    &	0.18&0.14	&	-0.02&0.02	&	0.30	&	0.07	&	0.06&0.10	&	0.05&0.15	\\
MKO	    &	0.07&0.00	&	0.22&0.43	&	0.31	&	0.02	&	-0.06&0.06	&	0.06&0.04	\\
ORM	    &	-0.40&0.06	&	-0.11&0.21	&	0.42	&	0.14	&	-0.02&0.01	&	0.07&0.15	\\
MDO	    &	0.33&0.11	&	0.02&0.02	&	0.03	&	0.01	&	0.01&0.00	&	0.08&0.19	\\
USA	    &	0.08&0.03	&	0.02&0.02	&	0.56	&	0.12	&	0.01&0.02	&	0.10&0.03	\\
DAG	    &	-0.08&0.01	&	0.05&0.24	&	-1.52	&	0.12	&	0.00&0.00	&	0.14&0.10	\\
BAO	    &	-0.11&0.10	&	0.01&0.00	&	2.45	&	0.31	&	-0.01&0.01	&	0.15&0.23	\\
SAO	    &	0.48&0.00	&	0.07&0.19	&	0.08	&	0.11	&	-0.02&0.02	&	0.16&0.00	\\
MRO	    &	0.11&0.04	&	-0.02&0.02	&	0.01	&	0.00	&	0.03&0.04	&	0.17&0.08	\\
\hline\hline
    \end{tabular}
    \label{T:regression}
\end{table*}

==> inc/old/w-tab_corr.tex <==
\begin{table*}
    \caption{%
    The statistical level of correlation corresponding to the correlation value.%
}
    \centering
    \begin{tabular}{lcc}
    \hline \hline
    Correlation Value & Relationship Level \\
    \hline \hline
    r  = 0 & No Relationship &  \\
    | r | < 0.20 & Very Weak Relationship &   \\
    0.20 < | r | < 0.39 & Weak Relationship & \\
    0.40 < | r | < 0.59  & Intermediate Relationship & \\
    0.60 < | r | < 0.79 & High Level Relationship & \\
    0.80 < | r | < 1.0 & Very High Level Relationship & \\
    \hline\hline 
    \end{tabular}
    \label{T:corr}
\end{table*}

==> inc/old/w-tab_normality.tex <==
\begin{table*}
    \centering
    \caption{%
    Normality test criteria and normality hypothesis for layers.
    }
    \begin{tabular}{l c c cc c cc}
    \hline \hline
Layer
    & Significance
    & Histogram
    & Skewness
    & Kurtosis
    & Q-Q Plot
    & Box Plot
    & Hypothesis Test
    \\
    \hline
CC
    & 0.00
    & +
    & -1.22
    & 1.52
    & +
    & +
    & h$_{0}$ refused 
    \\
PWV
    & 0.00
    & +
    & 1.80
    & 8.60
    & +
    & +
    & h$_{0}$ refused
    \\
AOD
    & 0.00
    & -
    & 1.15
    & 4.97
    & +
    & +
    & h$_{0}$ refused
    \\
WS1*
    & 0.00
    & +
    & 0.62
    & 4.05
    & +
    & +
    & h$_{0}$ refused
    \\ 
WS2*
    & 0.00
    & -  
    & 1.05 
    & 0.37
    & +
    & -
    & h$_{0}$ refused
    \\
DEM*
    & 0.00
    & -  
    & 1.96 
    & 3.77
    & +
    & +
    & h$_{0}$ refused
    \\  
LAT*
    & 0.00
    & -
    & -2.06 
    & 3.11
    & +
    & +
    & h$_{0}$ refused
    \\
    \hline\hline
    \end{tabular}
\label{T:normality}
 \end{table*}

==> inc/old/w-test.tex <==
\begin{table*}
    \begin{center}
        \begin{tabular}{*{10}{Z}}
          -1.00 & 1.00 & 1.00 & 1.00 & 0.99 & 0.98 & 0.96 & 0.90 & 0.82 & 0.37 \\
          1.00 & 1.00 & 0.99 & 0.98 & 0.95 & 0.90 & 0.82 & 0.61 & 0.37 & 0.01 \\
          1.00 & 0.99 & 0.98 & 0.96 & 0.90 & 0.82 & 0.67 & 0.37 & 0.14 & 0.00 \\
          1.00 & 0.98 & 0.95 & 0.90 & 0.78 & 0.61 & 0.37 & 0.08 & 0.01 & 0.00 \\
          0.99 & 0.95 & 0.90 & 0.82 & 0.61 & 0.37 & 0.14 & 0.01 & 0.00 & 0.00 \\
          0.98 & 0.90 & 0.82 & 0.67 & 0.37 & 0.14 & 0.02 & 0.00 & 0.00 & 0.00 \\
          0.95 & 0.78 & 0.61 & 0.37 & 0.08 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
          0.90 & 0.61 & 0.37 & 0.14 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
          0.82 & 0.37 & 0.14 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
          0.37 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        \end{tabular}
    \end{center}
\end{table*}

==> inc/w-fig7.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=\columnwidth]{fig/fig7/fig7.png}
\caption{%
Cross-correlation between two works: \citet{2019MNRAS.482.4941H} (y-axis) and this work (x-axis) for HWV.
The solid gray line represents y=0.816*x+4.33 and solid red line represents the best fit which corresponds R$^2$=0.95.%
}
\label{F:cor}
\end{center}
\end{figure}

==> inc/w-tabsup200W_monthly.tex <==
\begin{table*}
    \caption{%
    The monthly Wind Speed at 200 hPa of the observatories.
}
    \centering
    \begin{tabular}{lcccccccccccc}
    \hline \hline
    Observatories & Jan & Feb & Mar & Apr & May & Jun & Jul & Aug & Sep & Oct & Nov & Dec \\
    \hline
        SAAO &  26.76 &  25.83 &  25.29 &  25.00 &  28.75 &  34.72 &  35.70 &  37.24 &  35.33 &  31.40 &  29.63 &  28.00 \\
         CPO &  27.64 &  26.72 &  28.64 &  31.95 &  35.85 &  40.43 &  39.35 &  39.44 &  39.98 &  40.71 &  36.62 &  31.84 \\
        CTIO &  27.64 &  26.72 &  28.64 &  31.95 &  35.85 &  40.43 &  39.35 &  39.44 &  39.98 &  40.71 &  36.62 &  31.84 \\
         LCO &  26.09 &  25.79 &  28.21 &  32.11 &  36.00 &  40.23 &  39.47 &  38.96 &  40.07 &  40.51 &  36.71 &  31.35 \\
          CA &  16.92 &  17.46 &  21.34 &  29.90 &  34.72 &  37.42 &  37.46 &  34.94 &  36.43 &  34.88 &  31.48 &  24.86 \\
          PO &  16.94 &  17.42 &  21.28 &  29.66 &  34.39 &  37.02 &  37.00 &  34.48 &  35.94 &  34.56 &  31.28 &  24.80 \\
         MKO &  26.10 &  28.37 &  30.84 &  28.94 &  21.91 &  16.36 &  15.76 &  13.08 &  14.33 &  17.50 &  18.69 &  21.44 \\
         ORM &  20.41 &  23.68 &  27.23 &  30.06 &  27.61 &  19.92 &  12.93 &  12.44 &  16.33 &  15.45 &  17.63 &  19.11 \\
         MDO &  35.36 &  37.64 &  37.12 &  33.82 &  26.03 &  14.95 &   4.45 &   5.04 &  15.02 &  25.96 &  31.04 &  34.76 \\
        FLWO &  29.43 &  33.61 &  32.93 &  30.54 &  24.50 &  17.69 &   5.56 &   7.48 &  18.63 &  25.11 &  28.54 &  29.99 \\
        KPNO &  28.88 &  33.20 &  32.37 &  30.06 &  24.20 &  17.85 &   6.14 &   8.27 &  19.04 &  24.92 &  28.24 &  29.58 \\
        MGIO &  28.84 &  32.99 &  31.83 &  29.76 &  23.94 &  17.87 &   6.08 &   8.49 &  19.75 &  25.06 &  28.53 &  29.78 \\
        PalO &  25.30 &  29.36 &  28.41 &  25.82 &  21.32 &  18.36 &  11.29 &  13.72 &  20.53 &  21.77 &  24.56 &  25.81 \\
          LO &  26.12 &  30.09 &  28.39 &  26.70 &  22.00 &  18.82 &   9.75 &  13.17 &  21.48 &  23.28 &  27.08 &  27.62 \\
         DAG &  24.79 &  24.16 &  21.87 &  20.47 &  19.22 &  30.21 &  30.36 &  30.07 &  30.18 &  20.62 &  20.57 &  23.03 \\
         BAO &  38.30 &  37.63 &  36.20 &  32.74 &  31.10 &  25.81 &  23.86 &  24.90 &  34.67 &  35.60 &  36.02 &  36.61 \\
         SAO &  19.20 &  17.77 &  16.22 &  15.41 &  12.48 &  19.59 &  31.58 &  30.04 &  24.11 &  16.65 &  17.30 &  18.02 \\
         MRO &  23.92 &  20.11 &  19.38 &  17.87 &  15.48 &  17.00 &  19.74 &  17.21 &  18.95 &  25.20 &  27.42 &  24.82 \\
 
    \hline \hline
    \end{tabular}
    \label{T:200W}
\end{table*}

%okunan değerler kontrol edildi. trend benzerliği var. 


==> inc/w-tabsupAOD_monthly.tex <==
\begin{table*}
    \caption{%
    The monthly Aerosol Optical Depth of the observatories.
}
    \centering
    \begin{tabular}{lcccccccccccc}
    \hline \hline
Observatories & Jan & Feb & Mar & Apr & May & Jun & Jul & Aug & Sep & Oct & Nov & Dec \\
\hline
    SAAO &  0.20 &  0.20 &  0.19 &  0.22 &  0.20 &  0.20 &  0.20 &  0.22 &  0.26 &  0.22 &  0.23 &  0.21 \\
    CPO  &  0.43 &  0.34 &  0.24 &  0.24 &  0.31 &  0.58 &  0.82 &  0.90 &  1.06 &  0.68 &  0.36 &  0.40 \\
    CTIO &  0.34 &  0.28 &  0.24 &  0.24 &  0.27 &  0.41 &  0.50 &  0.52 &  0.60 &  0.40 &  0.36 &  0.33 \\
    LCO  &  0.36 &  0.30 &  0.28 &  0.26 &  0.29 &  0.40 &  0.52 &  0.52 &  0.48 &  0.38 &  0.34 &  0.30 \\
    CA   &  0.32 &  0.29 &  0.26 &  0.38 &  0.58 &  0.70 &  0.78 &  0.82 &  0.89 &  0.68 &  0.49 &  0.40 \\
    PO   &  0.77 &  0.59 &  0.52 &  0.61 &  0.68 &  1.09 &  1.25 &  1.30 &  1.22 &  1.23 &  1.04 &  1.03 \\
    MKO  &  0.57 &  0.73 &  0.96 &  0.92 &  0.86 &  0.78 &  0.61 &  0.57 &  0.80 &  0.55 &  0.46 &  0.34 \\
    ORM  & -0.45 &  1.06 &  1.56 &  1.69 &  1.76 &  1.70 &  2.25 &  2.06 &  1.64 &  1.20 &  0.94 &  0.86 \\
    MDO  &  0.25 &  0.26 &  0.29 &  0.34 &  0.40 &  0.66 &  0.90 &  0.92 &  0.62 &  0.37 &  0.30 &  0.23 \\
    FLWO &  0.21 &  0.24 &  0.23 &  0.26 &  0.31 &  0.36 &  0.64 &  0.75 &  0.58 &  0.40 &  0.30 &  0.22 \\
    KPNO &  0.24 &  0.27 &  0.34 &  0.36 &  0.41 &  0.47 &  0.72 &  0.64 &  0.59 &  0.36 &  0.26 &  0.24 \\
    MGIO &  0.24 &  0.29 &  0.38 &  0.44 &  0.51 &  0.50 &  0.66 &  0.55 &  0.48 &  0.30 &  0.24 &  0.24 \\
    PalO &  0.26 &  0.36 &  0.42 &  0.55 &  0.68 &  0.64 &  0.80 &  0.62 &  0.40 &  0.35 &  0.27 &  0.30 \\
    LO   &  0.38 &  0.39 &  0.53 &  0.30 &  0.34 &  0.48 &  0.60 &  0.49 &  0.34 &  0.33 &  0.34 &  0.31 \\
    DAG  &   NaN &   NaN &  3.36 &  2.46 &  1.02 &  0.87 &  0.90 &  0.92 &  0.64 &  0.60 &  0.60 &   NaN \\
    BAO  &  1.94 &  2.96 &  3.24 &  3.70 &  3.30 &  5.99 &  6.22 &  3.94 &  2.88 &  2.91 &  2.14 &  1.73 \\
    SAO  &  0.86 &  1.60 &  1.78 &  1.63 &  1.21 &  1.05 &  1.21 &  1.13 &  0.77 &  0.59 &  0.51 &  0.58 \\
    MRO  &  0.56 &  0.82 &  1.34 &  1.85 &  1.98 &  1.85 &  1.68 &  2.60 &  1.24 &  0.87 &  0.65 &  2.98 \\
    \hline \hline
    \end{tabular}
    \label{T:AOD}
\end{table*}

%okunan değerler kontrol edildi. Hellemeier makalesi datayı başka bir kaynaktan almış(toms data aerosol index) benzerlik yok. 
% dag degeri Nan ona bak


==> inc/w-tabsupCC_monthly.tex <==
\begin{table*}
    \caption{%
    The monthly Cloud Cover of the observatories.
}
    \centering
    \begin{tabular}{lcccccccccccc}
    \hline \hline
Observatories & Jan & Feb & Mar & Apr & May & Jun & Jul & Aug & Sep & Oct & Nov & Dec \\
\hline
    SAAO &  0.55 &  0.53 &  0.60 &  0.80 &  1.00 &  1.03 &  1.00 &  1.00 &  0.82 &  0.82 &  0.70 &  0.54 \\
    CPO  &  0.24 &  0.18 &  0.24 &  0.54 &  1.18 &  1.34 &  1.20 &  1.06 &  1.00 &  0.88 &  0.55 &  0.30 \\
    CTIO &  0.20 &  0.16 &  0.22 &  0.46 &  1.05 &  1.19 &  1.10 &  1.02 &  0.94 &  0.83 &  0.46 &  0.22 \\
    LCO  &  0.15 &  0.12 &  0.16 &  0.34 &  0.88 &  0.83 &  0.76 &  0.72 &  0.60 &  0.56 &  0.30 &  0.15 \\
    CA   &  0.30 &  0.26 &  0.08 &  0.20 &  0.42 &  0.49 &  0.37 &  0.21 &  0.17 &  0.16 &  0.08 &  0.15 \\
    PO   &  0.29 &  0.25 &  0.08 &  0.20 &  0.44 &  0.46 &  0.36 &  0.23 &  0.16 &  0.15 &  0.08 &  0.14 \\
    MKO  &  0.86 &  1.11 &  1.25 &  1.03 &  0.78 &  0.70 &  0.63 &  0.60 &  0.64 &  1.01 &  1.12 &  1.07 \\
    ORM  &  1.83 &  1.79 &  1.66 &  1.70 &  1.40 &  0.76 &  0.38 &  0.59 &  1.08 &  1.60 &  2.08 &  1.98 \\
    MDO  &  1.56 &  1.52 &  1.18 &  0.99 &  0.94 &  1.17 &  1.35 &  1.44 &  1.19 &  1.00 &  1.14 &  1.56 \\
    FLWO &  1.37 &  1.41 &  1.06 &  0.78 &  0.60 &  0.66 &  2.04 &  1.72 &  1.00 &  0.72 &  1.02 &  1.48 \\
    KPNO &  1.28 &  1.21 &  1.01 &  0.71 &  0.56 &  0.53 &  1.92 &  1.54 &  0.86 &  0.64 &  0.92 &  1.31 \\
    MGIO &  1.83 &  1.90 &  1.54 &  1.20 &  0.84 &  0.76 &  1.94 &  1.62 &  1.06 &  0.99 &  1.36 &  1.87 \\
    PalO &  1.55 &  1.64 &  1.32 &  1.08 &  0.84 &  0.39 &  0.62 &  0.48 &  0.45 &  0.74 &  1.14 &  1.54 \\
    LO   &  2.18 &  2.09 &  1.77 &  1.27 &  0.92 &  0.62 &  1.66 &  1.40 &  0.86 &  0.94 &  1.57 &  2.16 \\
    DAG  &  1.94 &  1.92 &  1.83 &  1.92 &  1.89 &  0.96 &  0.56 &  0.52 &  0.77 &  1.79 &  1.88 &  1.80 \\
    BAO  &  1.82 &  1.82 &  1.64 &  1.62 &  1.91 &  2.22 &  2.04 &  1.88 &  1.66 &  1.29 &  1.58 &  1.84 \\
    SAO  &  2.01 &  2.00 &  2.25 &  2.24 &  2.02 &  1.76 &  1.34 &  1.20 &  1.48 &  1.82 &  2.04 &  2.05 \\
    MRO  &  2.47 &  2.30 &  2.48 &  2.30 &  2.18 &  2.12 &  1.44 &  1.56 &  1.82 &  2.16 &  2.45 &  2.49 \\
    \hline \hline
    \end{tabular}
    \label{T:CC}
\end{table*}
% değerler kontrol edildi. 00=3, 01=2 10=1, 11=0 --> 3 hava bulutlu, 0 bulut yok.
% trend Hellemeier benzer fakat, Hellemeier değerleri 0-1 aralığına normalize etmiş. bizde yapabiliriz.


==> inc/w-tabsupPWV_monthly.tex <==
\begin{table*}
    \caption{%
    The monthly Precipitable Water Vapor of the observatories.
}
    \centering
    \begin{tabular}{lcccccccccccc}
    \hline \hline
Observatories & Jan & Feb & Mar & Apr & May & Jun & Jul & Aug & Sep & Oct & Nov & Dec \\
\hline
    SAAO &  13.77 &  14.36 &  12.64 &  10.22 &   8.52 &   5.93 &   5.67 &   5.78 &   7.20 &   9.15 &  10.18 &  11.64 \\
    CPO  &   9.29 &   8.93 &   8.33 &   7.22 &   6.93 &   6.06 &   5.38 &   5.52 &   5.31 &   5.68 &   6.18 &   7.18 \\
    CTIO &  11.14 &  10.71 &   9.88 &   8.59 &   8.09 &   7.06 &   6.04 &   6.34 &   6.02 &   6.48 &   7.21 &   8.64 \\
    LCO  &  10.20 &   9.84 &   8.86 &   7.81 &   7.36 &   6.80 &   5.80 &   5.84 &   5.73 &   6.28 &   6.58 &   7.55 \\
    CA   &  10.96 &  10.95 &   9.06 &   7.69 &   6.58 &   5.88 &   5.10 &   5.38 &   5.61 &   6.25 &   6.85 &   7.96 \\
    PO   &  13.57 &  13.70 &  11.59 &  10.02 &   8.75 &   7.98 &   6.89 &   7.30 &   7.48 &   8.14 &   8.71 &  10.03 \\
    MKO  &  11.34 &  11.41 &  11.36 &  11.70 &  13.44 &  15.36 &  16.23 &  16.76 &  16.12 &  15.52 &  13.34 &  11.56 \\
    ORM  &  13.92 &  13.38 &  14.18 &  15.19 &  17.40 &  21.54 &  28.60 &  30.48 &  26.65 &  21.88 &  17.43 &  14.57 \\
    MDO  &   6.10 &   6.28 &   7.34 &   8.53 &  12.70 &  19.42 &  24.22 &  24.07 &  18.38 &  11.07 &   7.40 &   6.22 \\
    FLWO &   6.70 &   6.42 &   6.84 &   7.41 &   9.87 &  15.74 &  28.18 &  25.84 &  18.37 &  10.55 &   7.99 &   6.86 \\
    KPNO &   7.76 &   7.34 &   7.96 &   8.72 &  11.74 &  17.70 &  31.34 &  29.33 &  21.52 &  12.74 &   9.19 &   7.80 \\
    MGIO &   6.09 &   5.88 &   6.28 &   6.98 &   9.21 &  14.68 &  26.42 &  23.55 &  15.48 &   9.33 &   7.04 &   6.28 \\
    PalO &   8.64 &   7.96 &   8.38 &   9.01 &  11.42 &  15.22 &  25.77 &  23.94 &  18.06 &  12.57 &  10.06 &   8.34 \\
    LO   &   4.22 &   4.44 &   4.96 &   5.52 &   7.44 &  10.43 &  19.74 &  17.50 &  11.62 &   6.98 &   5.52 &   4.99 \\
    DAG  &   2.07 &   2.14 &   2.58 &   3.90 &   5.48 &   7.38 &   8.04 &   8.85 &   6.69 &   5.64 &   3.52 &   2.45 \\
    BAO  &   3.67 &   4.20 &   5.91 &   9.09 &  13.26 &  20.58 &  30.70 &  27.05 &  16.10 &   9.81 &   6.22 &   4.19 \\
    SAO  &   3.66 &   3.81 &   4.66 &   6.14 &   8.80 &  12.13 &  14.10 &  14.26 &  10.51 &   8.03 &   5.88 &   4.46 \\
    MRO  &   6.38 &   6.14 &   6.72 &   7.97 &  10.77 &  14.02 &  16.76 &  16.88 &  14.51 &  10.40 &   6.86 &   5.92 \\
    \hline \hline
    \end{tabular}
    \label{T:PWV}
\end{table*}

==> inc/w-tabsupVW_monthly.tex <==
\begin{table*}
    \caption{%
    The monthly Vertical Wind Speed of the observatories.
}
    \centering
    \begin{tabular}{lcccccccccccc}
    \hline \hline
Observatories & Jan & Feb & Mar & Apr & May & Jun & Jul & Aug & Sep & Oct & Nov & Dec \\
\hline
        SAAO &  0.36 &  0.39 &  0.34 &  0.30 &  0.29 &  0.35 &  0.38 &  0.31 &  0.28 &  0.32 &  0.32 &  0.33 \\
         CPO &  0.09 &  0.13 &  0.25 &  0.37 &  0.40 &  0.39 &  0.37 &  0.42 &  0.40 &  0.36 &  0.27 &  0.14 \\
        CTIO & -0.05 &  0.01 &  0.16 &  0.38 &  0.61 &  0.83 &  0.85 &  0.76 &  0.54 &  0.36 &  0.18 &  0.01 \\
         LCO & -0.06 & -0.02 &  0.06 &  0.17 &  0.25 &  0.29 &  0.28 &  0.27 &  0.21 &  0.17 &  0.09 &  0.00 \\
          CA &  0.11 &  0.10 &  0.13 &  0.14 &  0.09 &  0.09 &  0.08 &  0.11 &  0.11 &  0.17 &  0.19 &  0.15 \\
          PO &  0.26 &  0.27 &  0.28 &  0.30 &  0.29 &  0.31 &  0.30 &  0.34 &  0.33 &  0.34 &  0.32 &  0.29 \\
         MKO &  0.38 &  0.33 &  0.25 &  0.25 &  0.24 &  0.22 &  0.19 &  0.16 &  0.17 &  0.18 &  0.21 &  0.33 \\
         ORM &  0.19 &  0.19 &  0.18 &  0.19 &  0.18 &  0.15 &  0.13 &  0.11 &  0.11 &  0.10 &  0.14 &  0.17 \\
         MDO &  0.21 &  0.10 & -0.00 & -0.06 & -0.17 & -0.23 & -0.20 & -0.18 & -0.17 & -0.10 &  0.13 &  0.26 \\
        FLWO & -0.05 & -0.10 & -0.18 & -0.23 & -0.28 & -0.30 & -0.17 & -0.08 & -0.08 & -0.14 & -0.10 & -0.04 \\
        KPNO & -0.04 & -0.14 & -0.27 & -0.33 & -0.37 & -0.44 & -0.35 & -0.29 & -0.34 & -0.35 & -0.16 & -0.01 \\
        MGIO &  0.01 & -0.07 & -0.15 & -0.28 & -0.45 & -0.50 & -0.27 & -0.24 & -0.25 & -0.21 & -0.04 &  0.01 \\
        PalO &  0.11 & -0.10 & -0.22 & -0.23 & -0.12 & -0.00 & -0.08 & -0.15 & -0.22 & -0.16 &  0.06 &  0.15 \\
          LO &  0.04 & -0.14 & -0.28 & -0.41 & -0.45 & -0.45 & -0.29 & -0.21 & -0.24 & -0.16 & -0.06 &  0.03 \\
         DAG &  0.17 &  0.14 &  0.13 &  0.11 &  0.08 &  0.06 &  0.03 &  0.01 &  0.04 &  0.11 &  0.14 &  0.16 \\
         BAO &  0.35 &  0.25 &  0.12 &  0.08 &  0.05 &  0.02 &  0.01 &  0.04 &  0.08 &  0.15 &  0.23 &  0.32 \\
         SAO &  0.53 &  0.43 &  0.37 &  0.26 &  0.17 &  0.08 & -0.00 &  0.04 &  0.15 &  0.26 &  0.39 &  0.51 \\
         MRO &  0.03 &  0.01 & -0.08 & -0.15 & -0.19 & -0.23 & -0.23 & -0.20 & -0.14 & -0.10 & -0.03 &  0.04 \\
    \hline \hline
    \end{tabular}
    \label{T:VW}
\end{table*}

==> name.tex <==
%According to Pearson and Spearman correlation, there is a moderate negative correlation between DEM-CC layers. There is a moderately negative correlation between DEM and PWV, according to the Spearman correlation. The weakest correlation between these two layers is the Kendall correlation. Fig. \ref{F:corr}, DEM-CC and DEM-PWV relationships are plotted. Observatories with a more cloudy sky than others are lower altitude observatories than others.Relationship between PWV and DEM Fig. \ref{F:corr}. As seen in Fig. \ref{F:corr}, it is an exponential relation. A similar result was made in \citet{2019PASP..131d5001O}'s study and it was concluded that the relationship between them is exponential. According to Pearson correlation, there is a moderate negative correlation between DEM-CC layers. According to the Spearman correlation, there is a moderately negative correlation between DEM-CC and DEM-PWV. The correlation coefficient where the relationship between the layers is the weakest is the Kendall correlation. In Fig.\ref{F:corr}, the graph of the relationship between AOD and CC layers is given in the second graph in the left column. According to the graph, as the amount of cloudiness increases, the amount of aerosol increases. When these aerosol particles are thought to be carried by clouds and help create precipitation, it is inevitable that there is a relationship between them.In the studies were analyzed, the relationship between many different parameters such as cloud fractions, cloud top height and cloud thickness, aerosol particle number and effective particle radius were examined and was observed that there was a correlation between AOD and CC \citep{2003JGRD..108.4699S}. Table \ref{T:coef} shows a moderate correlation in other correlations except the Kendall correlation.In the graphs associated with latitude at Fig.\ref{F:corr}, the effects in the northern and southern hemispheres are clearly visible. While AOD is less at low latitudes, the amount of AOD increases with increasing latitude. In this case, the amount of AOD increases as it moves away from the equator. In Table 5, where correlations are given, AOD-LAT is highly correlated for all three correlation coefficients, and this relationship is inverse.There is a moderate correlation between WS1 and AOD, as seen in all correlation coefficients. WS1 also showed a symmetrical effect with respect to the Equator. The reason for the increase of WS1 between latitudes of 25-45 compared to other latitudes is commercial winds and sub-tropical jet stream. Because of these air currents and trade winds, as one moves from the equator to the upper latitudes, the WS1 first increases and then decreases as it moves towards the polar cell.WS1 is lower in latitudes between 0-30, which are called Hadleyy cells, compared to mid-latitude cells.As can be seen in Table \ref{T:coef}, there is a moderate correlation in the CC layer. Especially in the middle latitudes, the cloud cover is higher than in the low latitudes.
